Foundation Model's Embedded Representations May Detect Distribution Shift

Sampling biases can cause distribution shifts between train and test datasets for supervised learning tasks, obscuring our ability to understand the generalization capacity of a model. This is especially important considering the wide adoption of pre-trained foundational neural networks -- whose behavior remains poorly understood -- for transfer learning (TL) tasks. We present a case study for TL on the Sentiment140 dataset and show that many pre-trained foundation models encode different representations of Sentiment140's manually curated test set $M$ from the automatically labeled training set $P$, confirming that a distribution shift has occurred. We argue training on $P$ and measuring performance on $M$ is a biased measure of generalization. Experiments on pre-trained GPT-2 show that the features learnable from $P$ do not improve (and in fact hamper) performance on $M$. Linear probes on pre-trained GPT-2's representations are robust and may even outperform overall fine-tuning, implying a fundamental importance for discerning distribution shift in train/test splits for model interpretation.

==> Adam_Tsou/notes.tex <==
% \documentclass{article}
% \usepackage{graphicx} % Required for inserting images
% \usepackage[top=0.5in, bottom=0.5in, left=0.5in, right=0.5in]{geometry}
% \usepackage{hyperref}
% \hypersetup{
%     colorlinks=true,
%     linkcolor=blue,
%     filecolor=magenta,      
%     urlcolor=cyan,
%     pdftitle={compbio},
%     pdfpagemode=FullScreen,
%     }

% \usepackage{listings}
% \usepackage{soul}
% \usepackage{xcolor}
% \usepackage{minted}

% %New colors defined below
% \definecolor{codegreen}{rgb}{0,0.6,0}
% \definecolor{codegray}{rgb}{0.5,0.5,0.5}
% \definecolor{codepurple}{rgb}{0.58,0,0.82}
% \definecolor{backcolour}{rgb}{0.95,0.95,0.92}

% %Code listing style named "mystyle"
% \lstdefinestyle{mystyle}{
%   backgroundcolor=\color{backcolour},   commentstyle=\color{codegreen},
%   keywordstyle=\color{magenta},
%   numberstyle=\tiny\color{codegray},
%   stringstyle=\color{codepurple},
%   basicstyle=\ttfamily\footnotesize,
%   breakatwhitespace=false,         
%   breaklines=true,                 
%   captionpos=b,                    
%   keepspaces=true,                 
%   numbers=left,                    
%   numbersep=5pt,                  
%   showspaces=false,                
%   showstringspaces=false,
%   showtabs=false,                  
%   tabsize=2
% }

% \title{Distributional Shifts Between Training and Test Data May Confound Learning}
% \author{Adam Tsou}
% \date{June 2023}

% \begin{document}

% \maketitle

% \begin{itemize}
%     \item Abstract - need to focus on 1 single topic
%     \item Introduction - What is the problem that we are studying? How has it been studied before? What have other people done? What do we do? Where is our added benefit to the field? We will follow up on prior work with a case study for Sentiment140. Introduce of baselines from random feature classification. Cite a bunch of papers on out of distribution performance/generalization (want to make the point that even though it can be contrived, its a problem of actual applied importance; OR there will already be a bunch of literature on this topic and we just cite cite cite).
    
%     \item Section 1 - Using local linearization of NN, we can perform EDA on the data. One such analysis is simply to plot the distribution of the distilled features of (previously seen/unseen) datasets. PCA on Sentiment140 clearly shows that the training data is intrinsically different from the test. This suggest that there is an artifact. (Can use PCA plots as well as densities)
%     \item Section 2 - What is the correct baseline to understand the magnitude and the effect of the artifact on Transfer Learning? We look at Random Feature Classification to understand how much information pre-trained GPT2 has on P and M. (Use the table here). \textcolor{red}{Somewhere around here, or before, we also should introduce the idea that Sentiment140 has this bias from just reading their paper.}
%     \item Section 3 - Understanding FT models via global FT vs linear FT. We extend the work of (cite the paper Adam found) to show that linear FT beats SOTA global FT. In this case, FT'ing on OOD P likely weakens the models ability to classify on M. (Is there a figure or a table we can use for this section?)
%     \item Conclusion - Not performing EDA such as we did can lead to confounding inference on FT models.
%     \item  Discussion - We can use local linearization to perform standard EDA and other Data Science 101 stuff. 
%     \item Put all other stuff in an oversized appendix
% \end{itemize}

% \section*{Relevant Papers}

% \subsection{Spectral evolution and invariance in linear-width neural networks}
% \begin{itemize}
%     \item Evolution of NN with LLM tends towards heavy-tailed spectra during FT. 
%     \item 1st PC aligns with sentiment but 2nd PC may not align with sentiment (correlation not necesarily causation). 
%     \item  Emergence of outlier eigenvalues lines up with feature learning. 
% \end{itemize}
% \subsection{Spectra of the Conjugate Kernel and Neural Tangent Kernel for Linear-Width Neural Networks}
% \begin{itemize}
%     \item CK evolves layerwise under random initialization with each subsequent layer being an MP map of the previous. Also shows evolution towards outliers with higher learning rate during training. 
% \end{itemize}
% \begin{subsection}{Layernorm}
% \begin{itemize}
%     \item Layernorm should have no adverse effects with minibatch size = 1. 
% \end{itemize}
% \begin{subsection}{A Kernel-Based View of Language Model Fine-Tuning}
% \begin{itemize}
%     \item CK and NTK are a model for LLM fine tuning both in prompt based tuning and conventional fine tuning. 
%     \item Not clear whether they are the correct model though. 
% \end{itemize}
% \end{subsection}
% \subsection*{Erhan et. al. 2010}
%     Pre-training acts as a regularizer, that favors hidden units that compute features that correspond to high variation in parameter space. 
% \subsection*{Dan Hendrycks 1 Kimin Lee 2 Mantas Mazeika}
%     Pre-training improves robustness to label corruption.

%     "pre-trained representations can transfer to a new task without adversarially tuning the entire network. In point of fact, if we only adversarially tune the last affine classification layer, and no other parameters, for CIFAR-10 and CIFAR-100 we respectively obtain adversarial accuracies of 46.6\% and 26.1\%".
% \subsubsection*{Jason Yosinski,1 Jeff Clune,2 Yoshua Bengio,3 and Hod Lipson4}
% Transfered weights perform better than random feature classification. Performance decreases with distance to target task. Transfer learning benefits stay after fine-tuning compared to a random feature model, and even for distant tasks.  
% \end{subsection}









% \end{document}

==> backup.tex <==
% \documentclass{article}

% %this has differnt options specified with
% %\usepackage[option]{neurips_2023}
% %I think they are [preprint] [final].
% \usepackage[preprint]{neurips_2023}
% \usepackage{comment}

% \usepackage{graphicx} % Required for inserting images
% %\usepackage[top=0.5in, bottom=0.5in, left=0.5in, right=0.5in]{geometry}
% \usepackage{hyperref}
% \usepackage{multirow}
% \usepackage{subfig}
% \hypersetup{
%     colorlinks=true,
%     linkcolor=blue,
%     filecolor=magenta,      
%     urlcolor=cyan,
%     pdftitle={compbio},
%     pdfpagemode=FullScreen,
%     }
% \usepackage{listings}
% \usepackage{soul}
% \usepackage{xcolor}
% \usepackage{minted}
% \usepackage{amsmath}
% %\usepackage{tikz}
% \usepackage{mathdots}
% \usepackage{yhmath}
% \usepackage{cancel}
% \usepackage{color}
% \usepackage{siunitx}
% \usepackage{array}
% \usepackage{multirow}
% \usepackage{amssymb}
% \usepackage{gensymb}
% \usepackage{tabularx}
% \usepackage{extarrows}
% \usepackage{booktabs}
% \usepackage{url}
% \usepackage{adjustbox}
% \usepackage{makecell}
% %\svgpath{{/Adam Tsou/imgs/}}

% \DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

% \newcommand{\inlinetodo}[1]{\textcolor{red}{\textbf{TODO:} #1}}
% \newcommand{\awecomment}[1]{\textcolor{olive}{\textbf{AE:} #1}}
% \newcommand{\tc}[1]{\textcolor{blue}{\textbf{tc:} #1}}
% \newcommand{\mv}[1]{\textcolor{orange}{\textbf{mv:} #1}}
% \newcommand{\gentodo}[2][]{\todo[linecolor=red,backgroundcolor=red!30,#1]{#2}}

% \newcommand{\FT}{\mathpzc{F}\hspace{0.005pt}\mathpzc{T}}
% \newcommand{\LP}{\mathpzc{L}\hspace{1pt}\mathpzc{P}}

% %New colors defined below
% \definecolor{codegreen}{rgb}{0,0.6,0}
% \definecolor{codegray}{rgb}{0.5,0.5,0.5}
% \definecolor{codepurple}{rgb}{0.58,0,0.82}
% \definecolor{backcolour}{rgb}{0.95,0.95,0.92}

% %Code listing style named "mystyle"
% \lstdefinestyle{mystyle}{
%   backgroundcolor=\color{backcolour},   commentstyle=\color{codegreen},
%   keywordstyle=\color{magenta},
%   numberstyle=\tiny\color{codegray},
%   stringstyle=\color{codepurple},
%   basicstyle=\ttfamily\footnotesize,
%   breakatwhitespace=false,         
%   breaklines=true,                 
%   captionpos=b,                    
%   keepspaces=true,                 
%   numbers=left,                    
%   numbersep=5pt,                  
%   showspaces=false,                
%   showstringspaces=false,
%   showtabs=false,                  
%   tabsize=2
% }



% \usepackage{booktabs}       % professional-quality tables

% \title{Distributional Difference Between Training and Test Data May Confound Inference On Transfer Learning}


% \author{%
%   \textbf{Adam Tsou}$^{1}$ \quad
%   \textbf{Max Vargas}$^{2}$ \quad \textbf{Andrew Engel}$^{2}$ \quad \textbf{Tony Chiang}$^{2,3}$\\
%   $^1$Stony Brook University \quad
%   $^2$Pacific Northwest National Laboratory \quad $^2$University of Washington\\
%   \texttt{\{adam.tsou\}@stonybrook.edu}\\
%   \texttt{\{max.vargas,andrew.engel,tony.chiang\}@pnnl.gov}
%   }



% \date{June 2023}

% \begin{document}

% \maketitle

% \begin{abstract}
%     %Understanding a learning algorithm's ability to generalize beyond the distribution of data used for training is critical to understand the success of \textit{transfer learning} (TL) in deep learning. \tc{We don't actually study the above at all.}
%     Distribution shifts between train and test datasets obscure our ability to understand the generalization capacity of neural network models. This topic is especially relevant given the success of pre-trained foundation models as starting points for transfer learning (TL) models across tasks and contexts. We present a case study for TL on a pre-trained GPT-2 model onto the Sentiment140 dataset for sentiment classification. We show that Sentiment140's test dataset \(M\) is not sampled from the same distribution as the training dataset \(P\), and hence training on \(P\) and measuring performance on \(M\) does not actually account for the model's generalization on sentiment classification. % In fact, we achieve $93.8\%$ accuracy simply by training a linear probe of the final embedding on a small sample of data from \(M\), outperforming full fine-tuning %confounds the model's ability to generalize on sentiment classification with the effects of the distribution shift. 
%     %We can observe this effect by comparing fine-tuned (FT) models with the \textit{correct} baseline models: a quantitative comparison with random feature regression models suggests that GPT-2 has an internal representation of sentiment, and that random feature (RF) regression is competitive with the fine-tuned model when training is performed on points that are from the same distribution as \(M\). 
%     In fact, we show that linear probes trained on the final embedding of pre-trained GPT-2 are surprisingly robust and are competitive with and may even outperform fine-tuning where all model weights update. This indicates that GPT-2's pre-existing representation of language is already able to classify sentiment.
% \end{abstract}

% %We start with a GPT-2's pre-trained weights and fine-tune (FT) on a limited dataset for a small number of epochs.

% \begin{section}{Introduction}
% % \inlinetodo{Need to write a high-level introduction to the part of ML that this research ties to. We can't start a paper like this. }
% % \inlinetodo{Andrew: A good introduction should be shaped like a funnel: very broad in topic and scope at first and quickly narrowing down to the specifics of the work and its importance. }

% % Andrew Engel's suggested Introduction outline:
% % \begin{enumerate}
% %  \item a short paragraph on The importance of transfer learning to the state of deep learning and foundation models in the year 2023
% %  \item The outstanding problems of transfer learning and the importance of solving them.
% %  \item Now narrow scope onto specifically this paper: one problem is that we do not always have access to data that is representative of the actual task we would like to solve. Instead, we use cheaper sampling / autonomous methods to collect lots of data that is more closely aligned with the ultimate task, but is not quite the task. The outstanding questions we want to answer are whether this practice is sound? And how do we avoid confounding the performance of our model via transfer learning and the distribution shift that has occurred?
% %  \item (Quickly say more about the methods you will use in your analysis if any of them warrant an introduction to a broad audience.) e.g., To answer this research question, we will draw on the recent advances from random matrix theory, and utilize random feature models as a baseline as suggested in cite{Pennington}, as well as well-known and time-proven methods like PCA. 
% % \end{enumerate}

% %Meaningful strides have been made in TL thanks to the remarkable advances in foundation models trained on vast amounts of data. 
% %Remarkable advances in foundation models has made transfer learning of podium importance. 
% Prototypical examples in transfer learning involve training on data with potential misalignment with the testing distribution. Such instances include training with machine-generated labels \cite{Radford2022RobustSR}, across geographical shifts, temporal drift, linguistic drift and more \cite{info:doi/10.2196/19273}. Due to distributional shifts, optimizations for the training distribution do not necessarily translate to optimizations on the testing distribution. If one starts with a foundation model that has already learned from a pre-training corpus, further training at the level of full fine-tuning 
% %adaptation to a task-specific training distribution 
% may not be necessary to achieve robust generalization \cite{Kumar2022FineTuningCD}, \cite{Zhou2023LIMALI}. We examine this possibility using random feature models \cite{Adlam2020UnderstandingDD} and linear probes \cite{Kumar2022FineTuningCD} as baselines, along with well-known and time-proven methods like PCA to show that foundation models may be readily able to discern distribution shifts and distill common textual features. % \awecomment{... to show that XXX and YYY?}

% %To address this question, we will utilize random feature models as a baseline as suggested in \cite{Adlam2020UnderstandingDD}, linear probes as in \cite{Kumar2022FineTuningCD}, as well as well-known and time-proven methods like PCA. %This raises the question, if models have already learned relevant features to a given task \cite{Zhou2023LIMALI}, can transfer learning weaken a model's ability to perform? %This is especially the case as models may have already learned relevant feature representations during pre-training \cite{Zhou2023LIMALI}. %In fact, pre-trained foundation models may already have performant capabilities on the downstream target task.

% %Some have gone so far to claim that a model's ability to solve these downstream tasks are largely developed in pre-training \cite{Zhou2023LIMALI}. Under this assumption, distributional shift between a training and testing set could weaken the performance of a model during transfer learning. 
% %A typical setting for transfer learning is one where we do not have training data that is representative of the task we would like to solve. Instead, we use cheaper sampling or autonomous methods to collect data that is more closely aligned with the ultimate task, but is not quite the task (cite). However, we are often in the case that the data distribution we care about 
 


% This paper is primarily a case study of Sentiment140 \cite{Go2009TwitterSC} and how an \textit{a priori} understanding of the distributional shift between its automatically processed training set ($P$) and manually curated testing set ($M$) via a selection bias allowed us to analyze the utility of full fine-tuning (FT) on a base model. 
% %The processed training dataset of Sentiment-140 (\(P\)) was generated by querying a series of emoticons matched to positive and negative sentiment labels. In contrast, the manually curated test dataset (\(M\)) was generated by querying from a list of 53 topics and labeled by human judges (\cite{Go2009TwitterSC}). Using emoticons as a proxy for sentiment is not a perfect, for example, as emoticons be used in a sarcastic manner that betray the sentimental intent of the author.\\
% We conduct a series of experiments to investigate the internal representations of $P$ and $M$ for the GPT-2 architecture, showing the surprising ability of the model to separate the distribution shift, and to leverage its pre-trained features for sentiment classification. We find:
% %Comparing fine-tuning or linear probes of a pre-trained model
% \begin{itemize}
%     %TL on distributionally mis-aligned training/test data leads to confounding inference on model generalizibility
%     \item[1.] Dimensionality reduction on the final embedding vector of GPT-2 can differentiate the distributional shift between datasets \(P\) and \(M\).
%     \item[2.] A linear probe (on pre-trained GPT-2) fit to a small sample of $M$ provides comparable performance for sentiment classification to state-of-the-art models which have been fine-tuned using $P$. This indicates that a model's ability to classify sentiment may be attributed to existing features learned in pre-training and not to features learned from $P$.
    
%     %relies on existing pre-trained features.
%     %\tc{This needs to be softened a bit...so let's think about clinical trials. If the treatment group is doing no better than control, then it's likely that are own immune system is taking care of the disease and the treatment is orthogonal to anything. We might be able to claim that FT on a few epochs isn't doing much and the classification after FT still relies on the pre-trained representations.}
    
    
%     %the performance of FT models trained on $P$ may largely rely on existing pre-trained features.
%     %For sentiment classification on $M$, state-of-the-art fine-tuned models transferred from learning on $P$ are outperformed by a linear probe trained on a small sample from \(M\) using the pre-trained features of GPT-2. %originally had `even on the entirety of dataset P??'
%    % \item[3.] Comparison against a random feature baseline for binary classification (as opposed to a `50/50' baseline) indicates that FT outperforms random 
%     %indicates FT on $P$ may harm performance on $M$.
%     %binary classification is more informative for assessing model generalizability than comparing with the `$50/50$' binomial baseline.
% \end{itemize}

% %If a NBA coach could go back in time, would s/he choose 1993 Michael Jordan or Jordan after he trained for one and a half years to do baseballs? One of the most common themes in machine learning is that training on data that is unsuitable for the task can adversely affect a model's performance, similar to how Michael Jordan's baseball training may have made him a worse basketball player. 

% %\quad In the domain sciences, the term "batch-effects" is used to refer to how small differences between experiments can compound, leading to data that varies significantly across repeated experiments with the same methodology. The same effect applies here in data science. Sentiment-140 was created as an easy way to model sentiment by using emoticons as a proxy for sentiment labels. It is composed of a manually sourced dataset and a processed dataset that uses emoticons as the sentiment labels. Although both datasets broadly reflect sentiment, the processed dataset is much more succeptible to confounders such as sarcasm. On the contrary, the manually sourced dataset was labeled by consensus from 3 human judges. As sentiment is a human endeavor, we would argue that the manually sourced dataset would be a better reflection of human sentiment than a dataset labeled on emoticons. 

% %\quad How to uncover such batch effects is a much more difficult question, and one that we will partially address by showing how we found distributional shifts between processed and manually curated data in Sentiment-140 via a linear model of the neural network feature space. By finetuning and evaluating on a split of the manually sourced data, we were able to achieve test accuracy that surpassed the current state of the art for Sentiment-140 over iid samples. These issues call for more principled baselines in finetuning foundation models. 
% \end{section}
% \begin{subsection}{Related Work}
% %\textbf{Conjugate Kernel}: The Conjugate Kernel (CK, NNGP) is the gram matrix of the outputs of the last hidden layer pre-non-linearity (activations). Building on work by (Neal, 1995), a wide body of literature (Cho and Saul, 2009, Hazan and Jaakola, 2015, Daniely et. al. 2016, Daniely 2017, Yang and Salman, 2019, Fan and Wang, 2022) associate the performance of wide randomly initialized neural networks to a gaussian process, relating that process to the conjugate kernel. 

% \textbf{Sentiment analysis} is a well studied task where the objective is to determine the emotional tone of a sequence of natural language \cite{Medhat:2014},\cite{d'Andrea:2015},\cite{Zhang:2018}, \cite{Radford2017LearningTG} \textit{et al}. 

% \textbf{Transfer learning} is most commonly applied by fine-tuning, where a randomly initialized task specific set of layers are appended to a pre-trained model. In full fine-tuning, all layers are allowed to update \cite{Yosinski2014HowTA}. Many large language models are pre-trained on self-supervised tasks like masked language completion, then evaluated on performance on a suite of downstream fine-tuning tasks \cite{Devlin2019BERTPO},\cite{Yang2019XLNetGA},\cite{Liu2019RoBERTaAR},\cite{Raffel2019ExploringTL},\cite{Wang2018GLUEAM},\cite{Go2009TwitterSC},\cite{Wang2019SuperGLUEAS},\cite{Maas2011LearningWV},\cite{Socher2013RecursiveDM} \textit{et al}. 

% \textbf{Linear probing} investigates the features associated with a layer by using its activation as an input feature vector to a linear classifier \cite{Belinkov2021ProbingCP}. A number of groups have studied linear probing: 1. for its explanatory uses \cite{Belinkov2021ProbingCP}, \cite{Alain2016UnderstandingIL}, \cite{Chen2020GenerativePF}, 2. to provide relative baselines \cite{Kumar2022FineTuningCD}, \cite{Rosenfeld2022DomainAdjustedRO}, and 3. for its relationship to zero-shot prompting \cite{Radford2021LearningTV}. In some cases, linear probing out-performs full fine-tuning \cite{Evci2022Head2ToeUI}. 

% \textbf{Random feature classification} is a form of linear probing on a random initialization of weights. Jarett \textit{et. al.} \cite{Jarett} was one of the first groups to pioneer a random feature baseline for vision models. A growing number of groups have established random feature baselines for language models, achieving surprisingly robust empirical results in language and sentiment analysis \cite{Conneau2017SupervisedLO}, \cite{Conneau2018WhatYC}, \cite{Zhang2018LanguageMT}, and addressed the challenge of establishing theoretical bounds for generalization \cite{Mei2019TheGE}, \cite{Yehudai2019OnTP}. 

% %Many large language models are pre-trained on self-supervised tasks like masked language completion, then evaluated on performance on a suite of downstream fine-tuning tasks (\cite{Devlin2019BERTPO},\cite{Yang2019XLNetGA},\cite{Liu2019RoBERTaAR},\cite{Raffel2019ExploringTL},\cite{Wang2018GLUEAM},\cite{Go2009TwitterSC},\cite{Wang2019SuperGLUEAS},\cite{Maas2011LearningWV},\cite{Socher2013RecursiveDM}) et al.

% %While many types of linear probes exist, we study linear probes of the last hidden layer. % Here, all model-weights are frozen and the final embedding vector of a model is flattened and used as an input feature vector for a linear model.

% %LP, in essence, learns a linear decision boundary that corresponds to the neural network's feature mapping (potentially random) while FT learns both an embedding of features as well as a linear decision boundary.

% %\subsection{Our Contributions} 


% \end{subsection}
% %We use RF in the same way as Jarrett et. al. \cite{Jarett}, providing a baseline for how a model would perform if no pre-trained features were inherited. We extend the work of 
% %Kumar et. al. \cite{Kumar2022FineTuningCD}  who compare linear probing and fine-tuning across distributional shifts. We study these shifts in natural language models where it is more difficult to determine whether data is in- or out-of-distribution of both the pre-training and adaptation datasets.

% %\inlinetodo{The following is some brainstorming:}

% %Things we want to consider: there have been studies (Mei 2019, Pennington 2020) that investigate random feature baselines very theoretically to explain "mysteries" in generalization such as double descent and generalization of in distribution to out of distribution data. They found that you can reproduce this with random feature regression so these "mysteries" should be expected behavior.  Conneau 2017/2018 compare LSTMs with random feature regression to a number of other NNs and achieve high accuracy. 

% %Kumar et al. 2022, Rosenfeld Ravikumar, Risteki 2022 consider a linear probe baseline off of pre-trained features. They argue that 1. ERM (supervized learning) is actually enough for a pre-trained model to help generalization for o-o-d. 2. linear probes can out-perform on out of distribution data, but should underperform to supervized fine tuning on in-distribution tasks. 

% %An analogy to why baselines are important and worth thinking about. Medical studies always consider treatments in comparison to a control treatment. For example, a clinical trial may want to compare two drugs A and B. Without a control to establish a proper baseline, an experiment comparing $A$ and $B$ will only measure relative effect. In particular, it may be the case that neither A nor B have beneficial effect. 
% % 

% %We advocate that foundational models such as GPT-2 already come equipped with a rich representation of natural language. In particular, our experiments indicate that a linear probe on GPT-2 is already able to classify sentiment on \(M\) with a handful of training data. Contrastingly, training on \(P\) worsens relative performance on \(M\), indicating that data coming from the distribution of \(M\) cannot be separated so readily. We expect this phenomena to not only apply to foundational models in NLP but also foundational models used throughout machine learning. In fact, we first experimented using finetuning and sequentially tested different methods until finally arriving at random feature classification.

% %In fact, we first tried to finetune GPT-2 directly using the data of \(P\) and evaluating on \(M\), naively expecting to see performance gains. However, subsequent tests indicated that these hopes were falsely led as linearly probing GPT-2 with data from \(M\) had better performance than full fine-tuning on \(P\). Moreover, testing with other models such as Falcon show that the representation spaces of pre-trained language models are able to distinguish the two datasets \(P\) and \(M\), hence indicating that their underlying distributions are distinct from one another.

% %This brings the point that machine learning practitioners ought to take greater emphasis on understanding their data and establishing proper baselines in order to evaluate their techniques.

% %Remarkable strides have been made in AI due to techniques that people have applied in the context of transfer learning. In this setting, we don't have access to training data which is representative to the distribution of interest. This opens the door to foundational questions on methodology. For example, how can we best measure performance of our models without having access to appropriate data? 

% %\end{subsection}

% \begin{section}{Methods} \label{sec:methods}
% %We analyze the CK of the pre-trained model and find that the processed and manually sourced dataset are separated in the PC space of the neural network's CK. A natural next question is what would you do if you assumed that the processed dataset was out of distribution to the manually sourced dataset? We probed this further and trained a random feature regression and a linear probe from the pre-trained model to differentiate between manually sourced and processed datasets, achieving 84 \% and 90 \% accuracy respectively.
% %Operating on the assumption that manually sourced and pre-trained datasets were separate distributions, we trained a linear probe on 300 points of the manually sourced dataset and evaluated on the remaining 59 over multiple iid samples, achieving a range of 89 \%to 98 \% accuracy. To compare, we finetuned GPT-2, training on the processed dataset and achieved 83 \% accuracy on the evaluation set. The highest reported accuracy for finetuned GPT-2 is 89.3 \% accuracy (papers-with code).
% %Finally, for a test of what would happen if GPT-2 was finetuned and evaluated on in-distribution data, we performed finetuning, random feature regression, and linear probing of 20,000 points of the processed dataset and evaluated on 20,000 additional points of the processed dataset, finding that finetuning had the highest validation accuracy when trained/evaluated in-distribution. 
% % All experiments listed in Table \ref{tab:MainComparison} were conducted on an Nvidia DGX-2 on a single A100-40 GPU using Python 3 via PyTorch \cite{Paszke2019PyTorchAI}. Due to memory limitations, we limited batch size to 1, while non-standard for full fine-tuning, still attained robust results. %In preliminary investigation, fine-tuning on A100-80 GPUs with a batch size of 8 also showed decreased accuracy compared to batch size of 1. 


% %\begin{subsection}{Problem Setup}\label{sec:prob-setup}
% %The case study in this paper has the following setup. In a typical data science setup, if datasets $X$ and $Z$ are pulled from the same distribution, then $f(x | Z)$ should generalize and perform well on $X$ so long as $f$ is trained well. In the transfer learning case, one naive intuition is that if $X$ and $Z$ come from 'expectedly similar' distributions, then $f(x | Z)$ should still perform respectably on $X$. The case study here negates this idea. If one uses even a small training set $X' \subset X$ ($|X'| << |Z|$), then $f(x | X')$ performs better on $X$ in comparison to $f(x | Z)$. In fact, comparison to past SOTA shows $f(x | Z)$ can frequently be outperformed by good baselines trained on $X'$ (i.e., RF). Additionally in our NLP setting, a model with a good general representation of language is able to distinguish the underlying distributions of $X$ and $Z$ from each other.
% %\end{subsection}  
% \begin{subsection}{Data Preparation}\label{sec:data-prep} % We obtained all data used in this experiment from the Stanford Sentiment-140 website \cite{S140website}. \inlinetodo{Emoticon/vs query needs to be in the introduction} The processed training dataset (\(P\)) was generated by querying a series of emoticons matched to positive and negative sentiment labels. In contrast, the manually curated test dataset (\(M\)) was generated by querying from a list of 53 topics and labeled by human judges \cite{Go2009TwitterSC}.\\
% All experiments utilize the Sentiment140 Dataset, a collection of tweets scraped from Twitter in the year 2009 \cite{Go2009TwitterSC}. The full dataset is comprised of an automatically processed dataset \(P\) and manually curated set \(M\). Here, \(P\) has 1,600,000 examples with labels inferred from sentimentally relevant emoticons scrubbed from the original tweets; for example ``:)'' indicates a positive tweet and ``:('' is negative. In contrast, \(M\) consists of 359 examples with human annotated sentiment labels. We note that some might view $P$ and $M$ as testing and training sets, respectively. We choose not to adopt this perspective for concern that $M$ and $P$ being drawn from different distributions.

% %Despite \(P\) and \(M\) originally being viewed as `training' and `testing' sets, we choose not to adopt this perspective instead viewing our experiments through the lens of transfer learning.% (i.e. that we can adapt the model on \(P\) or \(M\) to classify sentiment). % Crucial to the interpretation of our results, sentiment 140 was created using two distinct scraping methodology for constructing its intended training (\(P\)) and testing (\(M\)) datasets. The training set was scraped from twitter's API by searching for tweets containing sentimentally relevant emoticons and inferring labels from them; for example ``:)'' is labeled positive and ``:('' is labeled negative. Because the dataset can be labeled autonomously, the training dataset contains 1,600,000 many examples. In contrast, the test dataset was scraped from searches of Twitter's API from a small set of topics with and human annotated labels. The test dataset contains only 359 many examples.

% We sample either \(P\) or \(M\) for model training. In the first case, we generate a balanced subset of 20k points, a disjoint subset of 20k points for validation, and we evaluate on all of \(M\) (359 points). Call these sets $P_\text{train}$, $P_\text{val}$, and $P_\text{test}$, respectively. In the latter case, a similar approach generates sets $M_\text{train}$ and $M_\text{test}$; $M_\text{train}$ contains 150 of each class label and $M_\text{test}$ contains the 59 remaining samples for \(M\). %\tc{Great thing we found the bug or we would have had rotten egg on our face} 
% We emphasize that $M_\text{train}$ and $M_\text{test}$ contain no common data points. 

% %\textcolor{red}{Andrew's attempted math formalism-- neeed actual mathematician to check}. \mv{Unsure if the abstraction is necessary here, and I'm not convinced it's correct. It's a delicate thing to juggle what exactly is the population vs sample since everything seems drawn from S140 (which is also a sample of data..).} We will denote the population of tweets containing emoticons and automated sentiment labels as $\mathcal{P}$, and the population of tweets generated from the list of test-topics and human annotated labels as $\mathcal{M}$.

% %The datasets $P \subseteq \mathcal{P}$ and $M \subseteq \mathcal{M}$ are a sample drawn from each population. $P = \{(x_i,y_i),\ldots,(x_N,y_N) \}$ and $M = \{(x_i,y_i),\ldots,(x_T,y_T) \}$ \textcolor{red}{Note, I would have liked to use M as the length of the set M, but M is already taken. this brings up a good point: why have we named these sets P and M? What do they represent? or are they just arbitrary letters? Can we choose better?} \tc{I think it is just the way Sentiment140 labeled them as Processed and Manual}. In our experiments we also perform analysis using a validation set drawn from the population $\mathcal{P}$, $P_{\text{val}}$. Finally, we also use splits created from partitions from the dataset \(M\). Let $\tilde{M}$ and $\hat{M}$ be the partitions of the dataset \(M\), such that $\tilde{M} \bigcap \hat{M} = \varnothing$ and $\tilde{M} \bigcup \hat{M} = M$. \mv{The goal of this paragraph seems to try and establish notations. Probably a more direct way to do this.} 


% %\inlinetodo{Is the bias dataset really neccesary? We only mention it once in the results.}
% %Lastly, in order to understand the distributional shift (or bias) between \(P\) and \(M\), we create a dataset $(Bias)$ to train the model's ability to classify the selection bias of Sentiment-140. We choose 200 points from \(P\) and \(M\) respectively to form a training set (balanced by sentiment labels in both categories), and we test generalization on 160 points of \(P\) and 159 points of \(M\), also balanced by sentiment labels. % All data is pre-processed, according to the steps outlined in section 2.3 of the Sentiment 140 paper \cite{Go2009TwitterSC}.\\
% %State-of-the-Art (SOTA) benchmarks were obtained from Papers With Code \cite{PapersWithCodeS140}. 
% \end{subsection}

% \subsection{Pre-trained and Random Feature Neural Network Models}
% Our experiments use the GPT-2 architecture \cite{Radford2019LanguageMA}. For random feature classification, we initialize GPT-2 with random weights drawn from the truncated normal distribution $\mathcal{N}(0,0.02)$ 
% \cite{Radford2018ImprovingLU},\cite{Radford2019LanguageMA}. Otherwise, we use pre-trained weights from Hugging Face to initialize the transformer layers \cite{DBLP:journals/corr/abs-1910-03771}.% We also make use of random feature models based on a random initialization of the GPT-2 architecture, without pretraining. In our random feature models, the weight tensors of GPT-2 are initialized from the truncated normal distribution $\mathcal{N}(0,0.02)$ .

% %Our main set of experiments make use of the GPT-2 \cite{Radford2019LanguageMA} architecture. GPT-2 is a transformer decoder language model pre-trained on the WebText corpus for the self-supervised next-token completion language modeling task. The python library transformers (from Hugging Face) makes pre-trained weights available for download. We also utilize the GPT-2 architecture for ``random feature classification'' experiments. In these experiments we randomly re-initialize all the weight tensors of GPT-2 from the $\mathcal{N}(0, 0.02)$ distribution  

% %\inlinetodo{Should we send 2.2/2.4 to appendix?}
% %\begin{subsection}{Model}
% %We use GPT-2 and its associated tokenizer, obtained from Hugging-Face \cite{Radford2019LanguageMA}. We use a variant of the GPT-2 architecture, \textit{GPT2ForSequenceClassification}, which attaches a randomized linear head to the model, classifies on the activation of the last hidden layer for the last token, and changes the output of GPT-2 to logits. This model keeps the underlying GPT-2 architecture and also retains the standard pre-trained GPT-2 weights. One minor difference is that we add a bias layer to the linear head. The model internally computes a mean-squared error loss; we use \textit{BCEWithLogitsLoss}, however, to backpropagate the error using gradient descent. Inputs are tokenized and then masked with a max sequence length of 128. Inputs are not padded since we use a batch size of 1. 
% %\end{subsection}
% \subsection{Training} \label{sec:training}
% We use two different training methodologies in Section \ref{sec:results}. Further experiments in the Appendix deviate from the two methods listed here; more details can be found therein.
% \begin{itemize}
%     \item[$\mathpzc{F}\hspace{0.005pt}\mathpzc{T})$] Starting from pre-trained weights of GPT-2, we attach a randomly initialized linear head with a bias layer, and train for ten epochs, allowing \emph{all} weights to update. We use $P_\text{val}$ to choose an early stopping epoch. Evaluation is performed on $M$.
%     %We used the Adam optimizer with batch size 1, learning rate (lr) = $10^{-5}$ (selected after a sweep over learning rates), $\beta$-values 0.99 and 0.999, and $\epsilon = 10^{-8}$, and a linear learning rate decay scheduler \cite{Kingma2014AdamAM} 
%     \item[$\mathpzc{L}\hspace{1pt}\mathpzc{P})$] We perform linear probing for random feature and pre-trained initializations of GPT-2. We extract a feature vector at the final hidden layer and train a logistic regression classifier with training data $M_\text{train}$ for ten epochs. We use $M_\text{train}$ to determine an epoch to evaluate test accuracy on \(M_\text{test}\). 
%     % We used the Adam optimizer with batch size 1, learning rate (lr) = \(10^{-2}\) (selected after a sweep over learning rates), \(\beta\)-values .99 and .999 and $\epsilon = 10^{-8}$.
% \end{itemize}

% %\subsection{Linear Probing}
% %At the final hidden layer, we extract a feature vector and train a logistic regression classifier to training labels, minimizing the binary cross entropy loss function \cite{Alain2016UnderstandingIL}. 
% %This is equivalent to our experimental setup in which we freeze the model weights for all transformer layers after initialization, allowing only a randomly initialized linear head with a bias layer to update weights to minimize $L_{BCEWithLogits}$.
% %Linear probes are done subsequent to pre-trained and random initialization of GPT-2 (cf Appendix \ref{fig:LPdiagram}, \ref{fig:RFdiagram}). 
% %In performing a linear probe, we froze all layers except for the linear head's weight and bias layers, training for 10 epochs using Adam with batch size 1, learning rate (lr) = 1e-2 (selected after a sweep over learning rates), beta's at (.99, .999) and eps = 1e-8, and a linear learning rate decay scheduler \cite{Kingma2014AdamAM}. 
% % We select either first global maximizer of validation accuracy on \(P\) or the first global maximizer of training accuracy on \(M\) to determine an epoch to evaluate test accuracy

%  %\subsection{Fine-Tuning}
% %Starting from GPT-2 pre-trained weights, we attach a randomly initialized linear head with a bias layer for text sequence classification task. We perform full fine-tuning with Adam \cite{Kingma2014AdamAM}, allowing all model weights to update, minimizing  $L_{\text{BCE}}$ (see Appendix \ref{fig:ftGPTdiagram}). We selected the epoch to evaluate test accuracy in the same way as we did for linear probing.
% %\mv{I would like to see something like `We have three models based on the GPT-2 architecture ($X,Y,Z$). $X$ was trained using \(P\), $Y$ was trained using \(M\)...'. Right now this information is inside of some figure captions which is too condensed for me to follow}
% %

%  %\textbf{Pre-trained Model}: The pre-trained model was initialized with the GPT-2 weights from the Huggingface model configuration for all transformer layers while the head was randomly initialized. Subsequent training of the pre-trained model proceeds by either linear probing or fine-tuning. \\
%  %We also considered using SKLearn's LBFGS optimizer and forms of L2 regularization, and chose to use Adam for convenience. 

% %Fine-tuning was performed with Adam  with batch size 1, lr = 1e-5 (again selected by random sweep), beta's at (.99, .999) and eps = 1e-8, and a linear learning rate decay scheduler \cite{Kingma2014AdamAM}. In addition, we clipped the gradient at 1.0. We selected the epoch to evaluate test accuracy in the same way as we did for linear probing.
% %\subsection{Experiment Design}
% %<For the main results experiments, what specifically did you do? You should be able to state what you did using only terms/concepts that have been defined above; otherwise, that neccesitates introducing another section>. 


% %\begin{subsection}{Uncertainty Estimates} 
% %All experiments were run multiple times to ascertain both training and generalization variability. Seeds were manually set for the torch, numpy, and random modules. Experiments on \(M\) were performed 50x, with seeds 0-49, where \(M\) was shuffled with that specific seed, then split into training and evaluation sets. All other experiments were performed 10 times, with seeds 0-9, shuffling the data, then splitting accordingly. 
% %\end{subsection}
% \end{section}

% \section{Results}\label{sec:results}

% %Table~\ref{tab:MainComparison} captures three accuracy distributions for the experiments that we conducted to understand the effectiveness of FT GPT-2 relative to a LP on the RF as well as the pre-trained instance of GPT-2 (cf our experiments in section~\ref{sec:methods}).
% %We argue that both the random and pre-trained features obtained from GPT-2's architecture serve as highly informative relative baselines affording us a better understanding and interpretation for FT models. 



% %\begin{table}[!ht]
% %\centering
% %\caption{Accuracy and Comparison to Other Works}
% %\begin{tabular}{llll}
% %\toprule
% %Model & Training Accuracy & Validation Accuracy & Test Accuracy \\
% %\midrule
% % RF GPT-2 + LP (\(P\))   & $60.5 \pm 0.20$\% (\(P\))   & $59.6 \pm 0.14$\% (\(P\))&   $53.6 \pm 0.62$\% (\(M\))\\
%  %RF GPT-2 + LP (Bias) & $ 95.9  \pm 0.2$\%  (B) & --   &$86.9 \pm 0.8$\% (B)\\
% % RF GPT-2 + LP (\(M\)) &$85.8 \pm 0.32$\%  (\(M\))& --&  $80.2 \pm 0.66$\% (\(M\))\\
% % Pre-Trained GPT-2 + LP (\(P\))   & $77.3 \pm 0.1$\% & $76.4 \pm 0.09$\% &  $78.7 \pm 0.75$\% \\
% % Pre-Trained GPT2 + LP (Bias) &   $94.5 \pm 0.38$\%  & -- & $91.4 \pm 0.36$\% \\
%  %Pre-Trained GPT-2 + LP (\(M\))& $95.2 \pm 0.14$\%  & --   &$93.8 \pm 0.34$ \% \\
%  %FT GPT-2 (\(P\)) & $91.6 \pm 0.93$ \% & $83.5 \pm 0.09$ \% & $84.1 \pm 0.49 $\% \\
%  %FT GPT-2 + LP (Bias) & $93.4 \pm 0.28$ \% & -- & $92.3 \pm 0.64$ \% \\ 
%  %FT GPT-2 (\(M\)) &  $99.8 \pm 0.03$ \% & -- & $86.3 \pm 0.65$ \% \\
% % \\
% % \hline
%  %\hline
% % \\
% %  FT RoBERTa & -- & -- & $89.3$ \% \\
% %  FT ALBERT & -- & -- & $85.3$ \% \\
% % FT XLNET & -- & -- & $84.0$ \% \\ 
% %\bottomrule
% %\caption*{Table 1: Random Feature (RF) uses the GPT-2 architecture with weights randomly re-initialized from a truncated normal distribution. Linear Probing (LP) attaches a linear classification head to either a RF or a pre-trained model then only trains this head. Fine-tuning (FT) uses pre-trained GPT-2 allowing all weights to update. Training on \(P\) is done on a 20K subsample; Validation on \(P\) is for a disjoint 20K subsample of \(P\). Training on \(M\) is done on a 300 subsample, and testing on \(M\) is on the remaining 59 samples. Experiments on the models' ability to differentiate between the \(P\)/\(M\) bias (i.e. distributional shift) are also recorded. Values are shown plus or minus the standard error of the mean.}
% %\end{table}
% \begin{subsection}{LLMs can separate P and M with pre-trained weights}\label{sec:batch}  %Reduction of Fine-Tuned Model Generalization Likely Due to Disparate Distributions}\label{sec:batch}

% %Because \(P\) and \(M\) are sourced by fundamentally different methods, it is safe to assume that {\(P\)}-distribution is largely different from {\(M\)}-distribution. 


%     \begin{figure}[!ht]
%     \centering
%     %\subfloat[KDE of PC 1\label{subfig-2:KDE PC 1}]{%
%          % \includegraphics[width=.5\linewidth]{Adam Tsou/20k Training/pretrained1stPCPM.png}} 
%     \subfloat[KDE of PCs 1 and 2\label{subfig-1:KDE PCs 1/2}]{%
%           \includegraphics[width=.5\linewidth]{Adam Tsou/20k Training/pretrained1st2ndPCbias (1).png}}
%     \subfloat[Test Accuracy\label{subfig-2:test-accuracy}]{%
%           \includegraphics[width=.5\linewidth]{Adam Tsou/Random Feature/alltestaccuracies (14).png}}
%     \caption{(a) Kernel Density Estimate of the two largest principal components of the pre-trained final embedding representation of \(P\) and \(M\). %Kernel Density Estimates (KDEs) which plot an estimate of the probability density function of the values of the PCs of the pre-trained embedded kernel  corresponding to data from \(P\) and \(M\). %smoothed by a Gaussian kernel. 
%     (b) Normalized Histograms of generalization for different types of training and models, with state-of-the-art fine-tuned model performance shown as dashed lines for comparison\label{fig: distributions 1 and 2}}
%   \end{figure}
  
%  % \mv{interpretation/reorg: We examine the distributions of $P$ and $M$ through the lens of GPT-2. As \(P\) and \(M\) are sourced by different means, we hypothesize that \(P\) and \(M\) come from inherently different distributions of natural language. To investigate this hypothesis, we construct a local-linearization of GPT-2 to quantify how the neural network represents features from these datasets. This local-linearization comes from the embedded kernel --- the gram matrix of the activations of the last hidden layer prior to the linear head. PCA of this kernel, using the pre-trained weights of GPT-2, is able to separate $P$ and $M$ by only looking at the first two principal components. Figure \ref{fig: distributions 1 and 2} is strong evidence of our hypothesis. We believe that our exploratory data analysis through GPT-2 is an indicator that \(M\) is unsuitable to test generalization after training on \(P\). 
%   %\newline
%   %\newline
%  % Our techniques in this analysis follow those by Fort et. al \cite{Fort2021ExploringTL} who perform PCA of the embedded kernel to visualize out-of-distribution data; we extend their techniques for use with LLMs. Further experiments using linear classification to confirm the separability of $P$ and $M$ are available in Appendix Table: \ref{tab:BiasComparison}.}
  
%  %Given that \(P\) and \(M\) were sampled from different populations of tweets, a likely explanation for GPT-2's ability to separate \(P\) and \(M\) with pretrained features is that \(P\) and \(M\) inherently come from different distributions of natural language. We quantify how the neural network represents features from these populations by constructing a local-linearization of the neural network to plot the distribution of the distilled features of \(P\) and \(M\). PCA of the embedded kernel (the gram matrix of the activations of the last hidden layer prior to the linear head) was recently used by Fort et. al. (\cite{Fort2021ExploringTL}) to visualize out-of-distribution data, and we extend their work to LLMs. %Together, PCs 1 and 2 capture roughly $90\% $of the total explained variance of feature space. 
%  %\newline
%  %\newline
%  % In Figure \ref{fig: distributions 1 and 2} we show that GPT-2's pre-trained weights separate \(P\) and \(M\) by plotting the distributions of PC 1 and PC 2 of the pre-trained embedded kernel of GPT-2. Further experiments to confirm the separability of \(P\) and \(M\) with linear classifiers can be found in  Appendix Table: \ref{tab:BiasComparison}. The fact that GPT-2's weights separate \(P\) and \(M\) is enough to give us pause. We argue that \(M\) is unsuitable as a test set for generalization, as we know a priori that \(M\) is sourced by different means than \(P\). To use \(M\) as such could confound our interpretation of how the model performs.
  
%   %\inlinetodo{This sentence is going to cause us trouble. You do more than train 3 different linear classifiers in Table 2, so if you are going to reference that table, you will need to shore up the caption and write a section on each row of that table for the appendix. We should refer to the appendix section that describes all of the experiments as well so people won't be confused about just one big table.} 

%   We examine the distributions of $P$ and $M$ through the lens of GPT-2. As \(P\) and \(M\) are sourced by different means, we hypothesize that \(P\) and \(M\) come from inherently different distributions of natural language. To investigate this hypothesis, we construct a local-linearization of GPT-2 to quantify how the neural network represents features from these datasets. This local-linearization comes from the embedded kernel --- the gram matrix of the activations of the last hidden layer prior to the linear head. PCA of this kernel, using the pre-trained weights of GPT-2, is able to separate $P$ and $M$ by only looking at the first two principal components. Figure \ref{subfig-1:KDE PCs 1/2} is strong evidence of our hypothesis. We believe that our exploratory data analysis via GPT-2 may indicate that \(M\) is unsuitable to test generalization after training on \(P\). Table~\ref{tab:Confounders} (in the Appendix) shows a few data points from \(P\) that likely confound sentiment classification as intended (on \(M\)). %\tc{put some of the confounding tweets of P into appendix and reference it here.}. 
%   \newline
%   \newline
%   Our techniques extend those by Fort \textit{et. al.} \cite{Fort2021ExploringTL} (who perform PCA of the embedded kernel to visualize out-of-distribution data) to LLMs. Our additional  experiments using linear classification to confirm the separability of $P$ and $M$ are available in Appendix Table: \ref{tab:BiasComparison}.
  
%  \end{subsection}

% \begin{subsection}{Fine-tuning on datasets similar to M does not generalize to M}

% % \begin{table}[!ht]
% % \centering
% % \caption{Comparing Fine-Tuned GPT-2 with Targeted Linear Probes}
% % \begin{tabular}{llll}
% % \toprule
% % Model & Training Accuracy & Validation Accuracy & Test Accuracy \\
% % \midrule
% % Fine-Tuned GPT-2 \bfseries{(P)} & $91.6 \pm 0.93$ \% & $83.5 \pm 0.09$ \% & $84.1 \pm 0.49 $\% \\
% % Random Features GPT-2 + LP \bfseries{(M)} &$85.8 \pm 0.32$\%  & --&  $80.2 \pm 0.66$\% \\
% %  Pre-Trained GPT-2 + LP \bfseries{(M)} & $95.2 \pm 0.14$\%  & --   &$93.8 \pm 0.34$ \% \\
% % \bottomrule
% % \end{tabular}
% % \label{fig:ftGPT-2vsLP}
% % \caption*{\inlinetodo{The caption needs to give information on all the rows and all the columns. It seems like we don't ever talk about validation accuracy either in the caption nor in the main body of the text. If we keep it in the table, we should describe it in the caption, but if we never refer to it in the main body, we should get rid of it.} Table 1: {\bfseries{(P)}} indicates that the model was trained and validated on 20k subsamples of dataset \(P\), and evaluated on all $359$ points of \(M\). {\bfseries{(M)}} indicates that the model was trained on $300$ points of dataset \(M\) and evaluated on the remaining $59$ points of \(M\). Linear probing is abbreviated by (LP), and follows initialization. Values are shown plus or minus the standard error of the mean.}

% \begin{table}[!ht]
% \centering
% \caption{Comparing Fine-Tuned GPT-2 with Targeted Linear Probes}
% \begin{tabular}{llllll}
% \toprule
% Base Model & Method & Train Acc & Test Acc \\
% \midrule
% Pre-Trained GPT-2 & $\FT$ (fine-tuning) & $91.6 \pm 0.93$ \%   & $84.1 \pm 0.49 $\% \\
% Random Features GPT-2 & $\LP$ (linear probe) & $85.7 \pm 0.27$\%   & $57.8 \pm 1.05$\% \\
% Pre-Trained GPT-2  & $\LP$ (linear probe) & $95.3 \pm 0.15$\%    & $86.3 \pm 0.55$ \% \\
% \bottomrule
% \end{tabular}
% \label{fig:ftGPT-2vsLP}
% \caption*{Table 1: Those equipped with the $\mathpzc{F}\hspace{0.005pt}\mathpzc{T}$ method are fine-tuned using 20k datapoints from $P$ and tested on all 359 points of $M$. Those with the $\LP$ method have a linear probe trained using 300 points of $M$ and tested on the remaining 59 points of $M$. Values are shown $\pm$ the standard error of the mean.}
% %Random Feature (RF) uses the GPT-2 architecture with weights randomly re-initialized from a truncated normal distribution. Linear Probing (LP) attaches a linear classification head to either a RF or a pre-trained model then only trains this head. Fine-tuning (FT) uses pre-trained GPT-2 allowing all weights to update. Training on \(P\) is done on a 20K subsample; Validation on \(P\) is for a separate 20K subsample of \(P\). Training on \(M\) is done on a 300 subsample, and testing on \(M\) is on the remaining 59 samples. Values are shown plus or minus the standard error of the mean.
% \end{table}
%  From the perspective of transfer learning, we can ask: can one use information learned about $P$ to predict trends on $M$? The results in Table \ref{fig:ftGPT-2vsLP} indicate that this question is far more subtle than simply fine-tuning on $P$ and then predicting on $M$. Starting with a pre-trained GPT-2 model and using a small amount of data from $M$ to train a linear probe on the final hidden layer, one can separate the classes of $M$ with notable accuracy. With this as a point of comparison, changes in the model due to fine-tuning on $P$ are not reflected in sentiment classification on $M$. %On the other hand, any effects caused by fine-tuning the pre-trained model on $P$ are not reflected in the model's ability to separate classes of $M$ compared to the linear probe baseline. 

% %Linear probes were trained on a sample of \(M\), while fine-tuning was performed on a sample of \(P\) (see \ref{sec:data-prep}).  We outperform supervised fine-tuning on \(P\) with a linear probe on pre-trained GPT-2 (Table \ref{fig:ftGPT-2vsLP}).

% %\inlinetodo{I don't think that we should be highlighting the RF part of this paper anymore; it's not the take away point. It's incidental to the main points?? Move it to the discussion section where you talk more about RF?} 
% %This is significantly different from the na\"{\i}ve binomial baseline model for binary classification. 
% %The most striking statistics from Table~\ref{tab:MainComparison} are those related to the intrinsic differences between datasets \(P\) from \(M\) and to fitting a linear model on \(M\) from different feature spaces (i.e. from RF, Pre-trained, or FT). From the batch effect, we may infer that the intrinsic variation between \(P\)
% %from \(M\) largely overwhelms the variation between the sentiment classes (discussed in more details in Section~\ref{sec:batch}). 

% %The LP models trained solely on \(M\) also present interesting yet counter-intuitive results. For instance, a binary classification model trained on random features yields an average training accuracy of roughly $86\%$ (with over $90\%$ peak); this is expected for a highly over-parameterized model ($1.25$B in GPT-2) given only $300$ training points. The truly surprising result is the average test accuracy of roughly $80\%$ (with $89\%$ peak, cf Appendix Figure~\ref{fig:enter-RFD}) which implies that random feature sentiment classification generalizes. This is significantly different from the na\"{\i}ve binomial baseline model for binary classification. 

% %This indicates that transferring features from base GPT-2 by means of LP/FT only improves accuracy by \% from the RF baseline

% %\inlinetodo{Is the following sentence stating the obvious?} Comparison with the respective random feature models shows that both pre-trained LP and FT successfully transfer features from the base GPT-2 model. 

% %and that the advantage from pre-training is robust to distributional shifts, even across tasks (Processed, Bias, Manual).

%  %\begin{figure}
%    % \centering
%    % \centering
%    % \subfloat[Train Accuracy\label{subfig-1:train-accuracy}]{%
%    %       \includegraphics[width=.5\linewidth]{Adam Tsou/Random Feature/alltrainaccuracies (1).png}} 
%    % \subfloat[Test Accuracy\label{subfig-2:test-accuracy}]{%
%         %  \includegraphics[width=.5\linewidth]{Adam Tsou/Random Feature/alltestaccuracies (9).png}}
%     %\caption{Histograms of generalization for different types of training and models are presented. Discrete probability density functions are plotted, and state-of-the-art fine-tuned model instances are shown with dotted lines.}
%    % \label{fig:test-accuracies}
% %\end{figure}
% %textbf{Histograms of generalization for different kinds of transfer learning and model suggest ...}. LP Manual and RF manual were trained on 300 points of \(M\) and evaluated on 59 points of \(M\) with 50 training seeds. FT Processed was trained on 20,000 points of \(P\) and evaluated on 359 points of \(M\) over 10 different training seeds. Discrete probability density function for LP, FT, and RF, with the total probability for each histogram summing to 1 are rendered. Reported state-of-the-art FT language model instances, are shown by dotted lines.
% %\subsection[Linear Probes on sub-samples of M outperform state-of-the-art models trained on all of P]{Linear Probes on sub-samples of $\boldsymbol{M}$ outperform state-of-the-art models trained on all of $\boldsymbol{P}$}

% %\tc{We need to refactor the entirety of this paragraph now. Figure 8 says that LP(M) is statistically different from FT(P) and the QQ plots show a right skew for LP...hence if you want something with a higher accuracy on average, go with LP(M). Furthermore, we see a trend that increasing the number of training data points in M pushes test acc dist rightward in Fig 7, so rather than spend lots of money and time FT LLMs, it would be worth it even just to add a bit more higher quality data.}
% Figure ~\ref{subfig-2:test-accuracy} compares the distributions of test accuracies reported in Table \ref{fig:ftGPT-2vsLP}. Visually, the distribution for fine-tuning on $P$ is aligned with that of linear probing on $M$. Even the accuracy for a state-of-the-art transfer model on RoBERTa (trained on the entirety of \(P\)) overlaps with the distribution for pre-trained GPT-2 linear probes. Both the QQ-plot and a two-sided Kolmogorov–Smirnov test (\textit{p}-value of 0.007), however, show that the linear probes on $M$ differ on fine-tuning on $P$ (Figure~\ref{fig:distributiontests}). This suggests that  linear probes on $M$ may slightly outperform fine-tuning on $P$ (Figure \ref{subfig-2:test-accuracy}) in general.  At best, FT -- with a high cost in computation -- seems to have minimal effect on the pre-trained representations, and at worst, these observations indicate that the fine-tuning procedure may actually cause the model to forget relevant semantic information it had learned during pre-training.

% %In our sample, even the worst performing linear probe of a pretrained GPT-2 model scores better than the top performing random feature classifier. Moreover, it is visually clear that the distribution for fine-tuning on $P$ is better aligned with that of the random features baseline than for the linear probe. 

%   %Since linear probing outperforms fine-tuned GPT-2 as well as other reported state-of-the-art transfer models, in this case of Sentiment140 we observe that linear probing outperforms fine-tuning. This indicates that the fine-tuning procedure may actually cause the model to forget relevant semantic information it had learned during pre-training. 

% %\mv{This is something that is seen in a very visual way -- the blue distribution lines up more with purple than red.. how to say..} \tc{I agree, it's very intuitive when you look at the histograms, but we spend a crap ton of words not doing as well as simply saying "look at the figure".}
% %We interpret this in two ways: 1. the features of GPT-2 are expressive enough to be linearly separable, and 2. fine-tuning on \(P\) worsens the near optimal feature representation of GPT-2. 
%  %The accuracy distribution of linear probes on the pre-trained features of GPT-2 to be both higher and completely separate from that of linear probes on random features.



% %\begin{subsection}{Reduction of Fine-Tuned Model Generalization Likely Due to Disparate Distributions}\label{sec:batch}

% %Because \(P\) and \(M\) are sourced by fundamentally different methods, it is safe to assume that {\(P\)}-distribution is largely different from {\(M\)}-distribution.  


%  %   \begin{figure}[!ht]
%  %   \centering
%   %        \includegraphics[width=.5\linewidth]{Adam Tsou/20k Training/pretrained1stPCPM.png}} 
%   %  \hfill
%   %  \subfloat[KDE of PCs 1 and 2\label{subfig-3:KDE PCs 1/2}]{%
%   % %       \includegraphics[width=.5\linewidth]{Adam Tsou/20k Training/pretrained1st2ndPCbias (1).png}}
%    % \caption{Kernel Density Estimates (KDEs) which plot an estimate of the probability density function of the values of the principal components of the pre-trained embedded kernel (the gram matrix of the activations of the last hidden layer prior to the linear head) corresponding to data from \(P\) and \(M\), smoothed by a Gaussian kernel. \label{fig: distributions 1 and 2}}
% %  \end{figure}
% % Given that \(P\) and \(M\) were sampled from different populations of tweets, a likely explanation for GPT-2's ability to separate \(P\) and \(M\) with pretrained features is that \(P\) and \(M\) inherently come from different distributions of natural language. We quantify how the neural network represents features from these populations by constructing a local-linearization of the neural network to plot the distribution of the distilled features of \(P\) and \(M\). PCA of the embedded kernel (the gram matrix of the activations of the last hidden layer prior to the linear head) was recently used by Fort et. al. (\cite{Fort2021ExploringTL}) to visualize out-of-distribution data, and we adopt a similar analysis. %Together, PCs 1 and 2 capture roughly $90\% $of the total explained variance of feature space. 
% % \newline
%  %\newline
%  %We plot the distributions of PC 1 and PC 2 of the pre-trained embedded kernel of GPT-2, showing clear separation of distributions between \(P\) and \(M\) along the axis of the first principal component (cf Figure: \ref{fig: distributions 1 and 2}). \inlinetodo{This sentence is going to cause us trouble. You do more than train 3 different linear classifiers in Table 2, so if you are going to reference that table, you will need to shore up the caption and write a section on each row of that table for the appendix. We should refer to the appendix section that describes all of the experiments as well so people won't be confused about just one big table.} We confirm the separability of \(P\) and \(M\) by training 3 different linear classifiers to separate between \(P\) and \(M\) with between $86-92\%$ accuracy (cf Appendix Table: \ref{tab:MainComparison}). We argue that \(M\) is unsuitable as a test set for generalization given that the \inlinetodo{I would argue it's unsuitable because they are not the same distribution a priori. Otherwise, would you say it is OK to perform FT on P for Bert-base as the NN feature representation align??} neural network's feature representations of \(P\) and \(M\) differ significantly. To use \(M\) as such could confound inference on model performance. 

 
%  %This suggests that there are artifacts in Sentiment 140 generated by the sourcing of the data.
% %\subsubsection{Fine-tuned Models Largely Reside Within the Distribution of Random Feature Models}


% %We can actually say that the distribution of the LP and FT are quantatatively different since they only intersect at the single SOTA on RoBERTa. Because SOTA offer single points and not distributions, we argue that FT is quantatiatively no different than RF (since we can asusme that the SOTA are the outliers). 

% %%tc should move some of this stuff into the disscussion
% %We argue that RF on Manual provides suitable context for the generalization ability of FT on Processed as both train and test accuracy of distributions for FT on Processed and RF on Manual intersect. In contrast, the distribution of LP on Manual only intersects at one SOTA. Yehudai and Shamir \cite{Yehudai2019OnTP} formally link the performance of fine-tuning in vastly over-parameterized networks to the ability of random features to generalize, effectively showing that a random feature model can approximate polynomial decision boundaries, while fine-tuning allows for a more broad set of boundaries to be extracted from the feature representation. We observe that FT on Processed largely outperforms RF on Manual, therefore we can think of RF on Manual as giving a type of lower-bound on the generalization of FT. Most crucially, the worst accuracy of RF on M is more than 15\% better than 50\%, and while it is still not clear why this is the case, over-parameterization, size of the evaluation set, and implicit regularization by passing through the neural network are possible explanations. 

% \end{subsection}



% %\begin{section}{Discussion and Future Work}

% %\begin{figure}
%    % \centering
%    % {
%    % \includegraphics[width = .4 \linewidth]{Adam Tsou/PCA/BertBaseCased1st2ndPCbias.png}
%    % }
%    % {
%    % \includegraphics[width = .4 \linewidth]{Adam Tsou/PCA/RobertaBase1st2ndPCbias.png}
%   %  }
%   %  {
%  %   \includegraphics[width = .4 \linewidth]{Adam Tsou/PCA/falcon1b1st2ndPCbias.png}
%  %   }
%   %  {
%  %   \includegraphics[width = .4 \linewidth]{Adam Tsou/PCA/falcon7b1st2ndPCbias.png}
%   %  }
%   %  \caption{Kernel Density Estimates (KDEs) plotting the values of principal components 1 and 2 of the pre-trained embedded kernels for four different architectures for data corresponding to \(P\) and \(M\), smoothed by a Gaussian kernel.}
%   %  \label{fig:llms}
% %\end{figure}



% %One surprising statistic from our analysis comes from our RF baseline (roughly $80\%$ with $89\%$ peak). 

% %While prior work has shown that RF regression may give performance increases above na\"{\i}ve baseline models (\cite{Conneau2017SupervisedLO}, \cite{Conneau2018WhatYC}), this analysis showed \inlinetodo{we should make sure no one has published on something like this if we use this description} somewhat unprecedented generalization performance on a simple linear classification on \(M\). 

% %The truly surprising result is the average test accuracy of roughly $80\%$ for linear probing of GPT-2 initialized with random features (with $89\%$ peak, see Figure \ref{subfig-2:test-accuracy}, cf Appendix Figure~\ref{fig:enter-RFD}) which implies that random feature sentiment classification generalizes.

% %Prior work on infinite dimensional kernel support vector machines guarantees the linear separability of non-overlapping datasets (\cite{Chen2007OnLS}) which helps us better to understand RF training accuracy in highly over-parameterized settings, but not the generalization. This presents a new opportunity for AI research. 

% %And finally, we would like to address the issue of good and bad data. Good data will likely improve modeling for subsequent tasks. Bad data will likely add bias and confound the model. We want to stress that understanding the data, good or bad, is still useful for improving models. 

% %In fact, a priori understanding of the distributional shift from Sentiment 140 via a selection bias allowed us to analyze the utility of FT on a base model. In retrospect, using emoticons as a proxy for sentiment would add confounding effects due to sarcasm, typos, and even potential auto-corrections. Designing an experiment that can control for these effects is an essential component for modeling. 

% \begin{section}{Conclusions and Future Work}

% Much of the analyses in this case study can be generalized both to other models and datasets. We use four other pre-trained language models (Bert-base \cite{Devlin2019BERTPO}, RoBERTa-base \cite{Liu2019RoBERTaAR}, Falcon 1B, and Falcon 7B \cite{falcon40b}) to quantify the distributional shift between \(P\) and \(M\). Figure~\ref{fig:llms} shows that, while Bert-base cannot differentiate the shift, both RoBERTa-base and Falcon 1B can do so with limited success. Falcon 7B is able to completely differentiate the shift like GPT-2. This would suggest that the ability to differentiate the shift correlates with the number of parameters of the model, but this inference ignores other factors such as the training corpus for each language model. Our analysis cannot disentangle these confounding effects. Beyond analyzing other sentiment datasets, one natural way to extend this work is to generate sentiment labels by one LLM (e.g. GPT-4) and determine if we find a similar shift using a different LLM (Falcon 7B). 

% \begin{figure}
%     \centering
%     {
%     \includegraphics[width = .42 \linewidth]{Adam Tsou/PCA/BertBaseCased1st2ndPCbias.png}
%     }
%     {
%     \includegraphics[width = .42 \linewidth]{Adam Tsou/PCA/RobertaBase1st2ndPCbias.png}
%     }
%     {
%     \includegraphics[width = .42 \linewidth]{Adam Tsou/PCA/falcon1b1st2ndPCbias.png}
%     }
%     {
%     \includegraphics[width = .42 \linewidth]{Adam Tsou/PCA/falcon7b1st2ndPCbias.png}
%     }
%     \caption{Kernel Density Estimates (KDEs) plotting the values of PCs 1 and 2 of the pre-trained embedded kernels for four different architectures for data corresponding to \(P\) and \(M\). %smoothed by a Gaussian kernel.
%     }
%     \label{fig:llms}
% \end{figure}

% Our work has shown the unintended consequences when models are trained and subsequently evaluated on data from different distributions. This potentially leads the community to flawed inference on the performance of these models. 
% %and its capabilities to transfer knowledge to other domains. 
% These consequences can be challenging to ascertain in the absence of informative baselines for comparison. While our use of a linear probe baseline was specific to a classification task, other tools may be better suited to uncover the existing capabilities of pre-trained foundation models. The standard practice of either comparing with the na\"{\i}ve binomial/multinomial baseline models or benchmark models from prior studies may not be enough to fully understand the efficacy of trained models.
% %Training modern learners should still be viewed through the lens of conducting an experiment, and so providing a rigorous experimental design affords us better interpretation of the outcomes.  

% %\tc{Adam and I chatted; we should write two sentences about using GPT-4 to label sentiment to see if it does better than the automated methods here. We want to stress that we need to design the experiment via prompt engineering well so as to avoid confounding effects...TBD.}
% \end{section}


% %One concern this brings up is that finetuning on OOD data could in effect "sandbag" the pre-trained model, whereas fixing the features of the pre-trained model can lead to better performance. Another related concern is whether pre-trained models have memorized the target datasets. The list of scraped domains for GPT-2 includes Stanford (the creators of the dataset), and Github. We considered other approaches as well including clustering points in UMAP space based on their proximity to train and found that there was no meaningful difference when either cluster was used. 

% %Big picture: Three simple checks before performing TL using FT are presented. 1. Random feature baseline is much cheaper/reliable than other methods and can be repeated at scale, providing a principled baseline for model performance. 2. Few/Multishot Linear Probing can test the "quality" of a model's learned features, and "data efficiency" for higher scale transfer. 3. PCA of a feature space representation may reveal differences in the network's feature representations between subsets of a task dataset, and we use this to perform EDA as evidence of a distributional shift. Very simple steps that could save hundreds of dollars on a machine learning project.  

% %Look at other datasets/preprocessing steps to see if sourcing generates batch effects (pre-processing removing repeated letters is one example). Look at true few shot. Investigate random features through probing by looking at layer-wise representations. 
% %\end{section}






% \bibliographystyle{plain}
% \bibliography{main}

% \newpage
% \appendix
% \begin{section}{Experimental Details}
%  All experiments were conducted on an Nvidia DGX-2 on a single A100-40 GPU using Python 3.9, via PyTorch \cite{Paszke2019PyTorchAI}. Due to memory limitations, we limited batch size to 1, while non-standard for full fine-tuning, still attained robust results.

% \begin{subsection}{Uncertainty Estimates} 
% All experiments were run multiple times to ascertain both training and generalization variability. Seeds were manually set for the torch, numpy, and random modules. Experiments on \(M\) were performed 50x, with seeds 0-49, where \(M\) was shuffled with that specific seed, then split into training and evaluation sets. All other experiments were performed 10 times, with seeds 0-9, shuffling the data, then splitting accordingly. 
% \end{subsection}

% \begin{subsection}{Dataset and Model Sourcing}
% We sourced our data and models from openly available sources such as Hugging Face and Papers With Code. We obtained all training and evaluation data used in this experiment from the Stanford Sentiment140 website\footnote{http://help.sentiment140.com/for-students}. State-of-the-Art (SOTA) benchmarks were obtained from Papers With Code\footnote{https://paperswithcode.com/sota/text-classification-on-sentiment140}.  We used \textit{GPT-2ForSequenceClassification}, and \textit{GPT2Tokenizer} from Hugging Face for our experiments loaded from the Transformers Python library \cite{DBLP:journals/corr/abs-1910-03771}. 
% \end{subsection}

% \begin{subsection}{Pre-Processing Steps}
% We pre-processed text in Sentiment140 according to steps outlined in \cite[Sec 2.3]{Go2009TwitterSC}. Duplicate tweets were removed. In addition, we used regular expressions to find usernames, remaining emoticons, and URLs.  For example, a given username in a tweet would be converted to the token USERNAME. Likewise, a url would be converted to the token URL. Remaining emoticons were removed during our pre-processing.  
% \end{subsection}

% \begin{subsection}{Additional Experiments on Distributional Shift via Linear Classifiers} \label{sec:appendix bias linear probe}
% In order to understand whether \(P\) and \(M\) are linearly separable, we create a dataset $(Bias)$ to identify the model's ability to classify the selection bias of Sentiment140. We choose 200 points from \(P\) and \(M\) respectively to form a training set \(B_{\text{train}}\) (balanced by sentiment labels in both categories), and we test generalization on 160 points of \(P\) and 159 points of \(M\), also balanced by sentiment labels, \(B_{\text{test}}\).\\

% We perform linear probing for random feature, pre-trained, and fine-tuned initializations of GPT-2 training on the $(Bias)$ dataset. We train a logistic regression classifier with training data \(B_\text{train}\) for ten epochs. We use \(B_\text{train}\) to determine an epoch to evaluate test accuracy on \(B_{test}\).
% \end{subsection}

% \begin{subsection}{Additional Experiments on P and M}

% We list our full set of experiments in table~\ref{tab:MainComparison}, some of which were not highlighted in the main text.
% \newline
% \newline
% To understand the relative effect of training on $P$, we also test linear probes of random feature and pre-trained GPT-2 initializations. We take the same train/val/test split for sampling on $P$ as in \ref{sec:data-prep}, training on $P_{\text{train}}$, validating on $P_{\text{val}}$ and testing on $P_{\text{test}}=M$. 

% We additionally investigate whether fine-tuning on $M$ would overfit compared to a linear probe. We fine-tune on $M$, taking the same train/test split as described for sampling on $M$ in \ref{sec:data-prep}, training on $M_{\text{train}}$ and testing on $M_{\text{test}}$. Furthermore, we perform linear probing with samples of 100-250 points of $M$, increment by 50 per iteration and test on a held-out set of 59 points. Throughout, we use the same hyperparameters as in our original experiments in \ref{sec:training}.
% \end{subsection}

% \begin{subsection}{Hyperparameters}
% Hyperparameters used for all our experiments are shown in Table: \ref{tab:Hyperparameters}. \textit{BCEWithLogitsLoss} fuses a binary cross entropy loss and a sigmoid scaling operation. 
% \begin{table}[!ht]
% \centering
% \caption{Hyperparameters used in linear probing and fine-tuning}
% \begin{tabular}{llll}
% \toprule
% Hyperparameter & Linear Probing & Fine-Tuning \\
% \midrule
% Epochs & $10$ & $10$ \\
% Optimizer  & Adam & Adam \\
% Learning Rate & $10^{-2}$ & $10^{-5}$ \\
% $\beta_1$ & $.9$ & $.9 $ \\  
% $\beta_2$ & $.999$ & $.999$ \\ 
% $\epsilon$ & $10^{-8}$ & $10^{-8}$ \\ 
% Batch Size & $1$ & $1$ \\
% Scheduler-Type & LinearLR & LinearLR \\ 
% Start Factor & $.33$ & $.33$ \\
% End Factor & $1.0$ & $1.0$ \\
% Scheduler Iterations & $5$ & $5$ \\
% Dropout & $0.1$ & $0.1$ \\ 
% Gradient Norm Clip & $1.0$ & $1.0$ \\
% Seeds & $0-49$ for $M$, $0-9 $ otherwise & $0-49$ for $M$, $0-9$ otherwise \\ 
% Loss Function & BCEWithLogitsLoss & BCEWithLogitsLoss \\ 
% Random Feature Initialization  & \makecell[l]{Sample from $\mathcal{N}(0,0.02)$,\\ residual layers scaled by $\frac{1}{\sqrt{n}}$} & -- \\
% \bottomrule
% \label{tab:Hyperparameters}
% \end{tabular}
% \end{table}

% \end{subsection}
%     \begin{subsection}{Visualizing the Methods FT and LP}
%     Figures \ref{fig:ftGPTdiagram}, \ref{fig:LPdiagram}, and \ref{fig:RFdiagram} illustrate the experiments described in section \ref{sec:methods}. Specifically, figure \ref{fig:ftGPTdiagram} presents the typical transfer learning paradigm of learning on one dataset ($P$ in this case) and evaluating on a separate `expectedly similar' dataset ($M$). Figures \ref{fig:LPdiagram} and \ref{fig:RFdiagram} diagram attaching a linear head to examine feature representations for pre-trained and random feature initializations of GPT-2. 
%         \begin{figure}
%             \centering
%             \includegraphics[width = .7 \linewidth]{Adam Tsou/imgs/updatedft.drawio.png}
%             \caption{Full-fine-tuning of GPT-2, trained on a sample of P, evaluated on M}
%             \label{fig:ftGPTdiagram}
%         \end{figure}
%         \begin{figure}
%             \centering
%             \includegraphics[width = .7 \linewidth]{Adam Tsou/imgs/pretrainedlinearprobe.drawio.png}
%             \caption{Linear probe of pre-trained GPT-2, trained on a sample of M, evaluated on remainder of M.}
%             \label{fig:LPdiagram}
%         \end{figure}
%         \begin{figure}
%             \centering
%             \includegraphics[width = .7 \linewidth]{Adam Tsou/imgs/randomfeatureclassification.drawio.png}
%             \caption{Linear Probe of Random Feature GPT-2, trained on a sample of M, evaluated on the remainder.}
%             \label{fig:RFdiagram}
%         \end{figure}
%     \end{subsection}
% \end{section}
% \newpage
% \begin{section}{Examining P for Examples of Mislabeled Data}
% \begin{table}[!ht]
% \centering
% \caption{Possibly Mislabeled Data in $P$}
% \begin{tabular}{lllll}
% \toprule
% Label & ID  & Tweet \\
% \midrule
% :( & 1467863072 & \makecell[l]{@twitterhandle1}  \\ 
% :(& 1467871226 & \makecell[l]{@twitterhandle2 Congrats!! \\ i totally forgot to submit photos} \\ 
% :(& 1467979094 & \makecell[l]{@twitterhandle3 OHH! OMG. LMAO. \\ I'm crying right now, LOL! KUTNERRRR was the best!}  \\ 
% :) & 1836399555 & \makecell[l]{@twitterhandle4} \\ 
% :) & 1879932456 & \makecell[l]{@twitterhandle5 ????????????????} \\ 
% :) & 1833894264 & \makecell[l]{Just another SARS is coming...} \\ 
% \bottomrule
% \label{tab:Confounders}
% \end{tabular}
% \caption*{Table: 3 We present selected examples of potentially mislabeled in dataset $P$. The curators of Sentiment140 scrubbed the tweets in $P$ of emoticons. A ':(' corresponds to a 0 label, ':)' corresponds to 1 label.}
% \end{table}    
% In retrospect, using emoticons as a proxy to label sentiment is an imperfect method; one that the creators of Sentiment140 acknowledged as a key difficulty of creating their dataset \cite{Go2009TwitterSC}. Table \ref{tab:Confounders} showcases typical examples of such statements. Rows one and four consist of tweets only consisting of a social media handle after the relevant emoticon is removed. After pre-processing, the handle is changed to the token USERNAME, making these tweets a possible source of bias in the training data as inputs consisting of the exact same sequence of tokens would have opposite labels.
% \newline
% \newline
% Row two includes an example of mixed sentiment. One aspect of the tweet is positive ("Congrats!!"), yet one is negative "i totally forgot to submit photos", nevertheless a human annotator may label this tweet as positive considering it starts by mentioning another user's handle and congratulating them. Row three is arguably an example of a false-negative, and we believe that this sentence expresses positive sentiment. To us, row six shows a false-positive, referencing the spread of a disease. In its original context, with a smiling emoticon, the tweet in row six would have been an example of sarcasm. Row five is also a potential false-positive as a long sequence of question marks is traditionally associated with disbelief or anger. Given that $M$ was hand-labeled, we can assume that false-negatives and false-positives as shown in Table \ref{tab:Confounders} would not be as prevalent in the data. 
% \end{section}
% \begin{section}{Highlighting a Random Feature Baseline}
%   In their paper, Conneau et. al. \cite{Conneau2017SupervisedLO} demonstrate that linear probing of BiLSTM encoders initialized with random weights can achieve a peak of $80.7 \%$ accuracy in the SST-2 sentiment analysis dataset \cite{Socher2013RecursiveDM}. On our dataset, we average $57.8 \%$ test accuracy and reach $76\%$ peak as shown in Table \ref{fig:ftGPT-2vsLP} and Figure Appendix \ref{fig:enter-RFD}. We extend the work of Conneau et. al. \cite{Conneau2017SupervisedLO} with LSTMs to LLM models such as GPT-2 in our case study.

%  Recently, compelling work has been done investigating the generalization performance of random feature classification \cite{Mei2019TheGE}, \cite{Adlam2020UnderstandingDD}, \cite{Yehudai2019OnTP}. These are closely related to work on random initialization of neural networks as studied in \cite{Giryes2015DeepNN}. Daniely, Frostig and Singer \cite{Daniely2016TowardDU} show that with a random initialization, linear probing of the last hidden layer (equivalently last-layer training) can learn linear functions as well as more compliciated classes of functions obtained by non-linear kernel composition. These learning guarantees may be sufficient to achieve the generalization shown in our sentiment analysis task. In light of their work, studying random feature regression presents an exciting opportunity for AI research.
%  \end{section}

% \begin{section}{Additional Results}


% %\begin{figure}
% %    \centering
% %    {
% %    \includegraphics[width = .4 \linewidth]{Adam Tsou/PCA/BertBaseCased1st2ndPCbias.png}
% %    }
% %    {
% %    \includegraphics[width = .4 \linewidth]{Adam Tsou/PCA/RobertaBase1st2ndPCbias.png}
% %    }
% %    {
% %    \includegraphics[width = .4 \linewidth]{Adam Tsou/PCA/falcon1b1st2ndPCbias.png}
% %    }
% %    {
% %    \includegraphics[width = .4 \linewidth]{Adam Tsou/PCA/falcon7b1st2ndPCbias.png}
% %    }
% %    \caption{Kernel Density Estimates (KDEs) plotting the values of principal components 1 and 2 of the pre-trained embedded kernels for four different architectures for data corresponding to \(P\) and \(M\), smoothed by a Gaussian kernel.}
% %    \label{fig:llms}
% %\end{figure}


% \begin{table}[!ht]
% \centering
% \caption{Accuracy and Comparison to Other Works}
% \begin{tabular}{llll}
% \toprule
% Model & Training Accuracy & Validation Accuracy & Test Accuracy \\
% \midrule
% \\
%  RF GPT-2 + LP (\(P\))   & $60.5 \pm 0.20$\%   & $59.6 \pm 0.14$\% &   $53.6 \pm 0.62$\% \\
% Pre-Trained GPT-2 + LP (\(P\))   & $77.3 \pm 0.1$\% & $76.4 \pm 0.09$\% &  $78.7 \pm 0.75$\% \\
%  Pre-Trained GPT-2 + FT (\(P\)) & $91.6 \pm 0.93$ \% & $83.5 \pm 0.09$ \% & $84.1 \pm 0.49 $\%
%  \\ \\
%  \hline 
%  \\
%   RF GPT-2 + LP (\(M\)) &$85.7 \pm 0.27$\%  & --  & $57.8 \pm 1.05$\% \\
%  %Pre-Trained GPT-2 + LP (\(P\))   & $77.3 \pm 0.1$\% & $76.4 \pm 0.09$\% &  $78.7 \pm 0.75$\% \\
%  %Pre-Trained GPT2 + LP (Bias) &   $94.5 \pm 0.38$\%  & -- & $91.4 \pm 0.36$\% \\
%  Pre-Trained GPT-2 + LP (\(M\))& $95.3 \pm 0.15$\%  & --  & $86.3 \pm 0.55$ \% \\
% % FT GPT-2 (\(P\)) & $91.6 \pm 0.93$ \% & $83.5 \pm 0.09$ \% & $84.1 \pm 0.49 $\% \\
% % FT GPT-2 + LP (Bias) & $93.4 \pm 0.28$ \% & -- & $92.3 \pm 0.64$ \% \\ 
%  Pre-Trained GPT-2 + FT (\(M\)) &  $99.9 \pm 0.02$ \% & -- & $83.7 \pm 0.81$ \% \\
%  %RF GPT-2 + LP (Bias) & $ 95.9  \pm 0.2$\%   & --   &$86.9 \pm 0.8$\% \\
% %Pre-Trained GPT2 + LP (Bias) &   $94.5 \pm 0.38$\%  & -- & $91.4 \pm 0.36$\% \\
% %FT GPT-2 + LP (Bias) & $93.4 \pm 0.28$ \% & -- & $92.3 \pm 0.64$ \% \\ \\
% \\
%  \hline
%  \\
% RF GPT-2 + LP (Bias) & $ 95.9  \pm 0.2$\%   & --   &$86.9 \pm 0.8$\% \\
% Pre-Trained GPT2 + LP (Bias) &   $94.5 \pm 0.38$\%  & -- & $91.4 \pm 0.36$\% \\
% FT GPT-2 + LP (Bias) & $93.4 \pm 0.28$ \% & -- & $92.3 \pm 0.64$ \% \\
%  \\
%  \hline
%  \hline
%  \\
%   FT RoBERTa & -- & -- & $89.3$ \% \\
%   FT ALBERT & -- & -- & $85.3$ \% \\
%  FT XLNET & -- & -- & $84.0$ \% \\ 
% \bottomrule
% \label{tab:MainComparison}
% \end{tabular}
% \caption*{Table 4: Group one and two in the table are trained using data from $P$ and $M$, respectively. They are both evaluated using testing data from $M$. The third grouping is trained and tested on the Bias dataset described in \ref{sec:appendix bias linear probe}. The final group are state-of-the-art (SoTA) fine-tuned model instances described on the online repository Papers With Code.} %Random Feature (RF) uses the GPT-2 architecture with weights randomly re-initialized from a truncated normal distribution. Linear Probing (LP) attaches a linear classification head to either a RF or a pre-trained model then only trains this head. Fine-tuning (FT) uses pre-trained GPT-2 allowing all weights to update. Training on \(P\) is done on a 20K subsample; Validation on \(P\) is for a disjoint 20K subsample of \(P\). Training on \(M\) is done on a 300 subsample, and testing on \(M\) is on the remaining 59 samples. Experiments on the models' ability to differentiate between the \(P\)/\(M\) bias (i.e. distributional shift) are also recorded. Values are shown plus or minus the standard error of the mean.}
% \end{table}    

% \begin{figure}
%     \centering
%     \includegraphics[width = .7 \linewidth]{Adam Tsou/Random Feature/allrfaccuracies (2).png}
%     \caption{Training and Test Accuracy of a linear probe on the random features from GPT-2 architecture, trained on a held-out sample of 300 points from $M$, evaluated on the remainder.}
%     \label{fig:enter-RFD}
% \end{figure}
% \begin{subsection}{Linear Probes separate P and M with high accuracy}
%    \begin{table}[!ht]
% \centering
% \caption{Linear Probes of the $(Bias)$ dataset}
% \begin{tabular}{llll}
% \toprule
% Base Model & Training Accuracy  & Test Accuracy \\
% \midrule
%  Random Features GPT-2 & $ 95.9  \pm 0.2$\%   &$86.9 \pm 0.8$\% \\
%  Pre-Trained GPT-2 &   $94.5 \pm 0.38$\%  & $91.4 \pm 0.36$\% \\
%  Fine-Tuned GPT-2 & $93.4 \pm 0.28$ \% & $92.3 \pm 0.64$ \% \\ 
% \bottomrule
% \label{tab:BiasComparison}
% \end{tabular}
% \caption*{We present linear probes from three different initializations trained to classify whether a tweet belonged to either $P$ or $M$. Our models were trained on $B_\text{train}$, and evaluated on $B_\text{test}$ from the $(Bias)$ dataset described in \ref{sec:appendix bias linear probe}.}
% \end{table}   
% Expanding on our exploratory analysis in \ref{sec:batch}, we trained a series of linear classifiers to determine if tweets belonged to either $P$ or $M$ according to the experimental setup described in \ref{sec:appendix bias linear probe}. Our results show that even a linear probe off of random features was able to perform this task with $86.9 \%$ accuracy as shown in \ref{tab:BiasComparison}. Moreover, we see that probes of the pre-trained and fine-tuned models can separate the distribution shift with even greater accuracy.
% \end{subsection}
 
% \begin{subsection}[Training on P under-performs on P compared to M]{Training on $\boldsymbol{P}$ under-performs on $\boldsymbol{P}$ compared to $\boldsymbol{M}$}

% Using GPT-2's pretrained feature representations to examine $P$ and $M$ gives a surprising result. The validation accuracies on $P_\text{val}$ in rows 2 and 3 of Table \ref{tab:MainComparison} are lower than the testing accuracies on $M$. This result should give us pause by itself, since we typically expect the generalization metric to be lower than the training metric. This is especially the case with using $P$ and $M$ as training and testing distributions since our bias experiments indicate that $P$ and $M$ are linearly separable, hence are drawn from different distributions. We conjecture that the data of $M$ is more closely aligned to the pre-training corpus of GPT-2, than the data of $P$. Consequentially, one might view sentiment classification on $P$ as a more out-of-distribution task than sentiment classification on $M$. 

% When these results are interpreted in context with the linear probe baseline of pre-trained GPT-2 on \(M\), we deduce that training on \(P\) may bias sentiment classification on \(M\) (also supported from the RF+LP on \(P\), row 1 of Table~\ref{tab:MainComparison}). Additionally, FT models on \(M\) show a clear overfit onto the training data (near $100\%$) with a substantial drop-off for test accuracy (approximately $83\%$).
% \end{subsection}
% \begin{subsection}{Training with more data on M leads to increased average performance}
% \begin{figure}
%     \centering
%     \includegraphics[width = .7 \linewidth]{Adam Tsou/Last Layer/lptestaccuracieskde (2).png}
%     \caption{KDE plots of test accuracy for linear probes trained on 100/150/200/250/300 points of $M$ and tested on 59 points in the remainder of $M$}
%     \label{fig:sample-size-lpm}
% \end{figure}
% Figure \ref{fig:sample-size-lpm} presents KDEs and means of the distributions of test accuracy for linear probing on varying size samples of $M$. As the sample size increases, we see a clear rightward trend. Moreover, going from 100 points to 300 points gives a relative gain of roughly $8 \%$. If this trend were to continue past 300 points, we could potentially see linear probe models with higher average test accuracy than existing state-of-the-art models.  
% \end{subsection}
% \begin{subsection}{FT on M and LP on M are not the same distribution}
% \begin{figure}
%     \centering
%     \includegraphics[width = .7 \linewidth]{Adam Tsou/Last Layer/qqLPvsFT.png}\\
%     \includegraphics[width = .7 \linewidth]{Adam Tsou/Last Layer/KStest.png}
%     \caption{A QQ plot and a 2-sided KS test of test accuracies for linear probes of pre-trained GPT-2 and fine-tuned GPT-2 on M are presented.}
%     \label{fig:distributiontests}
% \end{figure}
% The QQ plot for the quantiles of the test accuracies for LP on $M$ (on the x-axis) against FT on $P$ (on the y-axis) implies differing distributions with a larger dispersion for test accuracies of linear probes fit.  Moreover, applying a 2-sided KS test returns a \textit{p}-value of 0.007, showing that the distributions of fine-tuned models and linear probe models are likely not the same. 
% \end{subsection}
% \end{section}


% %We believe that this is because while the model has been adapted to classify on P, M is still in-distribution of the original pre-training corpus. Therefore, evaluating on M is in-distribution with the features of the original GPT-2 model. 
% \end{document}
